Business Process Deviance Mining: Review and Evaluation

Business process deviance refers to the phenomenon whereby a subset of the executions of a business process deviate, in a negative or positive way, with respect to its expected or desirable outcomes. Deviant executions of a business process include those that violate compliance rules, or executions that undershoot or exceed performance targets. Deviance mining is concerned with uncovering the reasons for deviant executions by analyzing business process event logs. This article provides a systematic review and comparative evaluation of deviance mining approaches based on a family of data mining techniques known as sequence classification. Using real-life logs from multiple domains, we evaluate a range of feature types and classification methods in terms of their ability to accurately discriminate between normal and deviant executions of a process. We also analyze the interestingness of the rule sets extracted using different methods. We observe that feature sets extracted using pattern mining techniques only slightly outperform simpler feature sets based on counts of individual activity occurrences in a trace.

==> rulesinterestingnesseval_-_backup.tex <==
\section{Rules Interestingness Evaluation}\label{sec:RulesInterestingnessEval}

We inducted rules from the six datasets across seven feature types using decision tree classifier. This technique takes a leaf node of the decision tree as a rule. All decision trees are trained with uniform input parameters. As a result, there are seven rulesets for each dataset. The rule has the form of $A=>B$, where the antecedent A is a conjunction of multiple selectors in the form of \textit{attribute OP value} with \textit{OP} as relational operator, and the consequent B is the class label.

For each dataset, we compare the quality of these rulesets on a number of selected measures and observe the effect of pattern types on the rules quality. The measures used in our evaluation include:

\begin{itemize}
	\item Rule Length: the number of operators in the antecedent part of the rule. This is averaged from all rules of a ruleset.
	\item \%Generalization \cite{gallion1993dynamic}: the generalizability based on the number of training examples and the number of rules.
		\begin{equation}\label{eq:generalization}
		\%Generalization = (1 - \frac{\# of Rules}{\# of Training Examples})*100
		\end{equation}
	\item Probability-based Objective Rule Interestingness Measures. \cite{Geng2006} evaluates 38 interestingness measures with reference to 12 desired properties. The authors ranked these measures in terms of how much they hold a property (Table $V$ in \cite{Geng2006}). Based on this evaluation, we were able to select six top measures as listed below (noted that Yule's Q and Yule's Y are normalized variants of Odd Ratio \cite{tan2004select}). Readers should refer to \cite{Geng2006} for a detailed discussion on these measures while a brief description is given below.
	\begin{itemize}
		\item Collective Strength ($CS$): proposed in \cite{aggarwal98collective} to replace the support-based paradigm in frequent itemset mining. The original idea is to measure the collective strength of an itemset $I$ as $CS(I) = \frac{Good Events}{E[Good Events]}*\frac{E[Bad Events]}{Bad Events]}$, where \textit{Good Events} are when the items in the itemset are found in most of transactions and \textit{Bad Events} are when they are not. In the context of rule evaluation, \textit{Good Events} are when A and B are strongly correlated, and the opposite are \textit{Bad Events}. The collective strength $CS$ ranges from 0 to $+\infty$. If $CS=0$, A and B are mutually exclusive (perfect negative correlated). If $CS=1$, A and B are totally independent. If $CS$ increases to $+\infty$, A and B are increasingly positive correlated. 
		
		\begin{equation}\label{eq:collectivestrength}
		CS = \frac{P(AB)+P(\neg B|\neg A)}{P(A)P(B)+P(\neg A)P(\neg B)}*\frac{1-P(A)P(B)-P(\neg A)P(\neg B)}{1-P(AB)-P(\neg B|\neg A)}
		\end{equation}
		
		\item Two-Way Support ($TWS$): proposed in \cite{yao97twoway} to search for interesting knowledge through multiple databases. The knowledge in search has a similar form of a rule. This measure ranges from $-\infty$ to $+\infty$. If it approaches $+\infty$, the relation $A=>B$ increases and vice versa, the relation $B=>A$ increases when it approaches $-\infty$.
		
		\begin{equation}\label{eq:twowaysupport}
		TWS = P(AB)*\log_2\frac{P(AB)}{P(A)P(B)}
		\end{equation}
		
		\item \(\phi\)-Coefficient: has been used in statistics which is based on Pearson correlation coefficient. The coefficient range is between -1 and +1. When it is greater than 0, A and B are positively correlated. When it equals 0, A and B are independent. When it is less than 0, A and B are negatively correlated.
		
		\begin{equation}\label{eq:phicoefficient}
		\phi-Coefficient = \frac{P(AB)-P(A)P(B)}{\sqrt{P(A)P(B)P(\neg A)P(\neg B)}}
		\end{equation} 
		
		\item Piatetsky-Shapiro ($PS$): originally proposed in \cite{piatetsky91rules}, reflects the variance of probability when A and B are correlated and independent, with values ranging from -0.25 and 0.25. If PS is zero, A and B are totally independent. If PS is greater than 0, A and B are positive correlated, and vice versa, less than 0 when A and B are negative correlated. 
		
		\begin{equation}\label{eq:piatetsky}
		PS = P(AB) - P(A)P(B)
		\end{equation}
		
		\item Yule's Q ($YuleQ$): a normalized version of Odds Ratio ($OR$) which was proposed in \cite{mosteller68odds}, and based on the contingency table involving A and B. It measures the degree to which A and B are associated with each other. Yule's Q ranges from -1 (pefect negative correlation) to +1 (perfect positive correlation).
		
		\begin{equation}\label{eq:oddsratio}
		OR = \frac{P(AB)P(\neg A\neg B}{P(A\neg B)P(\neg AB)}
		\end{equation}
		
		\begin{equation}\label{eq:yulesQ}
		YuleQ = \frac{OR-1}{OR+1}
		\end{equation}
		
		\item Information Gain ($IG$): related to the Lift measure $\frac{P(AB)}{P(A)P(B)}$, i.e. how many times it needs to lift the confidence from the case when A and B are totally independent $P(A)P(B)$ to the case when A and B are statistically correlated $P(AB)$. IG ranges from $-\infty$ (negative correlated) to $+\infty$ (positive correlated).
		
		\begin{equation}\label{eq:informationgain}
		IG = log\frac{P(AB)}{P(A)P(B)}
		\end{equation}
		
	\end{itemize}
\end{itemize}	

\subsection{Patterns and Rules}\label{PatternsAndRules}
In this section, we review patterns and rules extracted from each dataset. A qualitative assessment is necessary to understand the insight of the rulesets and their context.

Evidently, across datasets and feature types, we noted that those patterns with high Fisher score are often chosen to form high-coverage rules. This is justifiable because the Decision Tree would pick up these patterns as preferable splitting points due to their strong discriminative power (Gini index is used for Decision Tree in our experiment). We observed that the higher Fisher score a pattern achieves, the more rules they may involve and the higher coverage those rules are.

Specifically, for the Schedule dataset, IP detects a remarkable pattern: "364 198 361" (sequence of software execution events). In the ruleset, there is also a high-coverage rule involving this pattern: \textit{IF "364 198 361" $\geq$ 0.500 THEN failing}, which means if this pattern occurs in the trace, that trace would have a failing outcome. In comparison with the IA-based ruleset, we noted that there are not any rules that involve the similar structure based on these three events. This means Decision Tree over IAs cannot detect such sequences and their correlation with the trace outcome.

For the MySQL dataset, IP and MR detect a few patterns with extremely high Fisher scores. Consequently, IP-based and MR-based ruleset contain only two rules involving the identified patterns. In the context of this dataset, the trace execution will fail if the pattern appears in the trace ("9 16 17 19 24 26 28 56 60 68 70 72 75 78 88" for IP and "c9b4j7i3b5i2l2d0f0e8j0d6" for MR - every two consecutive letters represent one event). We also noted that there are no rules generated for IA, TRA and SET using the same rule generation parameters (all features have highly equal values).

For the Hospital1 dataset, the IA dominates the feature selection list with much higher Fisher scores than the composite patterns (0.292 vs. 0.05), which is observed throughout all feature types. We noted that there is one top activity in the feature list ("Nursing Progress Notes") with score of 0.292 while the rest of the list are ranked at much lower range (approximately 0.05 and below). Across feature types, the selected list of patterns contains a balanced mix of composite patterns and IAs. As a result, most rulesets have a high-coverage rule based on "Nursing Progress Notes" and many low-coverage rules based on mix of composite patterns and IAs. In particular to this chest pain treatment process, with the temporal deviance outcome criterion, it seems that "Nursing Progress Notes" activity plays a determinant role in relation to the case duration. If there are more "Nursing Progress Notes", the case would last longer and vice versa.

For the Hospital2 dataset, we noted the same phenomenon as the Hospital1, that the IA dominates the feature selection list. Only IP and SET can provide patterns with the same Fisher score as the IA. Another remarkable characteristic of this process is most of the traces are short (about 5-6 events per cases - see Table~\ref{tab:datasets2}) which is already an indication that repetition of activities is rare. This phenomenon makes sense: a patient assessment process involved sending the patient to one or more medical personnel (who are generally not specialists) to assess the dominant mental health issue(s) and, subsequently, the right type of specialist to see. As a result, during the assessment process, patients are not likely to come back to see the same medical personnel more than once. That's why there are very few MR, MRA, TR and TRA patterns. %\colorbox{yellow}{SURIADI: PLEASE ADD YOUR COMMENTS}.

For the Insurance1 dataset, IP and MR result in some remarkable patterns. For example, some selected IP patterns are \{"New Claim, Authorise Payment, Close File", "New Claim, Close File", "New Claim, Generate Payment, Close File", "New Claim, Generate Payment, Authorise Payment, Close File", "New Claim, Authorise Payment", "Conduct File Review, Follow Up Requested"\}. Some MR patterns are \{"Conduct File Review, Follow Up Requested"\}. We can see that the IP patterns have covered the MR patterns since IP mines sequences of both consecutive and non-consecutive events. For example, for "New Claim, Authorise Payment, Close File", "New Claim" only occurs at the start of a case and "Close File" only occurs at the end. This differs from the MR patterns where the activities are adjacent to each other. Let's review one representative rule: \textit{IF "New Claim, Authorise Payment, Close File" $\leq$ 0.5 AND "New Claim, Close File" $\leq$ 0.5 THEN Long Case} (coverage: 28\%). This rule can be interpreted that if the case is not closed with an authorized payment, it is likely to be a long case. However, in the IA-based ruleset, we noted that there are also very similar rules involving "New Claim", "Close File" and "Generate Payment", as well as "Conduct File Review" and "Follow Up Requested". The reason is that the selected feature list of IA contains these activities with equivalent Fisher scores as the composite patterns. There are several IP-based patterns with slightly higher scores, for example "1 13 16" (0.344 vs. 0.159) and "1 16" (0.292 vs. 0.159). That's why IP could have a marginally better prediction than other features but could not surpass the IA. In other words, IA carries most of the signal related to the process outcome.

For Insurance2 dataset, IP and SET provides frequent patterns with higher Fisher scores than the IA and other patterns. Some example IP patterns are: "New Claim, Process Additional Information", "Process Additional Information, Contact Customer", "Process Additional Information, Conduct File Review". Example SET patterns are: "Conduct File Review, New Claim, Process Additional Information", "New Claim, Process Additional Information", "New Claim, Contact Customer, Process Additional Information", "Conduct File Review, New Claim, Contact Customer, Process Additional Information". Let's take a look at a high-coverage rule extracted from the IP-based ruleset: \textit{IF "Process Additional Information, Contact Customer" $\geq$ 0.5 THEN Rejected Case} (51\% coverage). This rule means if "Process Additional Information" and "Contact Customer" occurs, the case is likely rejected. The implication is that if the officer finds any anomalies in the claim application and s/he does contact the customer to verify, the claim would face a likelihood of being rejected. In comparison with the IA-based ruleset, we noted that the IA-based ruleset also has rules involving "Process Additional Information" and "Contact Customer" but also involving other activities which lengthens the rule. This is because, individually, "Process Additional Information" and "Contact Customer" rank very high in IA but lower than the composite patterns of IP and SET.

Our conclusion from the above analysis is that individual activities likely carry most of the outcome-related signals in case of temporal deviance outcome criterion. This has been reflected through our review of the content of the selected feature list for each feature type and datasets, as well as evidenced in the way rules are formed by the Decision Tree. Composite patterns, from our above observation, can contribute some interesting frequent patterns from qualitative perspective, which not only explains the dataset (in case of highly structured processes), but also make rule more concise and meaningful. 

\subsection{Rules Interestingness Measures}

We use different metrics to asssess the quality of rulesets. Rule Length is computed by averaging the length of all rules in the ruleset. \%Generalization is computed according to the formula (\ref{eq:generalization}). For Coverage, Support and the Probability-based Objective Measures, we computed the cumulative interestingness by firstly sorting the rules within one ruleset in decreasing magnitude of the interestingness measures, then accumulating the measure value from the highest to lowest. The cumulative measures represent the variation in interestingness of a ruleset based on the number of best rules chosen. All measures are then depicted in graphs and charts by datasets as shown in the Appendix section.

We draw the following observations from reviewing the graphs and charts for each dataset.

For the Schedule dataset, the IP-based ruleset has consistently high interestingness over the others, except in \(\phi\)-Coefficient where the TR and TRA are the best. Notably, IP-based ruleset also achieves the highest predictive outcome, as well as TR and TRA. Rule Length and \%Generalization are quite similar across feature types.

For the MySQL dataset, the IP-based and MR-based ruleset apparently show the best trend of cumulative interestingness, which accords closely with their absolutely high predictive strength. They also have the shortest length and the greatest \%Generalization. We noted there are no rules generated for IA, TRA and SET using the same rule generation parameters.

For the Hospital1 dataset, the MRA-based and IP-based ruleset achieve the higher cumulative values than the others in all measures except the Coverage. They also have high \%Generalization after the IA-based. However, all rulesets have very equal length.

For the Hosptal2 dataset, all rulesets are highly balanced across interestingness measures, rule length and \%Generalization. This equivalence corresponds to their equal predictive power and Fisher score as reviewed in section \ref{sec:AccuracyEvaluation} and \ref{PatternsAndRules}.

For the Insurance1 dataset, the IP-based and MRA-based rulesets are often placed higher than the others in different measures while the Set-based is the highest for Coverage. The IP-based and Set-based also have slight improvement over others in terms of Rule Length and \%Generalization.

For the Insurance2 dataset, we observed that the MRA-based is cumulatively better than the others in most of the measures, including the Rule Length and \%Generalization, except in \(\phi\)-Coefficient, Yule's Q and Information Gain where the Set-based seems to be the highest.

In summary, across all datasets, we observed that the IP-based, MRA-based and Set-based ruleset are often at the top range of the cumulative interestingness measurement. The IP-based often results in shorter length and higher \%Generalization in some datasets. The IA-based ruleset is often below the others in most of the measures, except in Yule's Q and Information Gain where it only improves when there are many more rules included. Though the rulesets based on composite patterns generally could not predict better than the baseline in weakly structured processes, the objective interestingness measures show that they may embed interesting aspects that are worth a further examination by business analysts.




